Selection, Ensemble, and Adaptation: Advancing Multi-Source-Free Domain Adaptation via Architecture Zoo

Conventional Multi-Source Free Domain Adaptation (MSFDA) assumes that each source domain provides a single source model, and all source models adopt a uniform architecture. This paper introduces Zoo-MSFDA, a more general setting that allows each source domain to offer a zoo of multiple source models with different architectures. While it enriches the source knowledge, Zoo-MSFDA risks being dominated by suboptimal/harmful models. To address this issue, we theoretically analyze the model selection problem in Zoo-MSFDA, and introduce two principles: transferability principle and diversity principle. Recognizing the challenge of measuring transferability, we subsequently propose a novel Source-Free Unsupervised Transferability Estimation (SUTE). It enables assessing and comparing transferability across multiple source models with different architectures under domain shift, without requiring target labels and source data. Based on above, we introduce a Selection, Ensemble, and Adaptation (SEA) framework to address Zoo-MSFDA, which consists of: 1) source models selection based on the proposed principles and SUTE; 2) ensemble construction based on SUTE-estimated transferability; 3) target-domain adaptation of the ensemble model. Evaluations demonstrate that our SEA framework, with the introduced Zoo-MSFDA setting, significantly improves adaptation performance (e.g., 13.5% on DomainNet). Additionally, our SUTE achieves state-of-the-art performance in transferability estimation.

==> table/tab_greedy.tex <==
\begin{table}
\caption{Classification accuracies (\%) under Zoo-MSFDA setting in Office-Home dataset. $\rightarrow$R denotes the tasks A, C, P$\rightarrow$R.. Avg. denotes the average accuracy. Top$_n$ indicates selecting the Top$_n$ most transferable models to establish $S_{TR}$.}
\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline
 Method & $\rightarrow$R & $\rightarrow$P &$\rightarrow$C & $\rightarrow$A & Avg. \\
\hline
Top$_2$ & 93.5 & 94.8 & 82.7 & 92.5 &90.8 \\
Top$_3$ & 94.4 & 95.0 & 83.9 & 92.6 &91.5 \\
Top$_5$ & 94.3 & 93.9 & 82.5 & 91.5 &90.5 \\
Top$_{10}$ & 93.1 & 95.3 & 75.8 & 87.0 &87.8\\
Ours(greedy) & 95.2 & 95.3 & 83.7 & 92.8 & 91.8 \\
%Ours(tc.)+nrc&&94.9&95.2&84.0&92.7&\\
\hline

\end{tabular}
%}
\label{tab_greedy}
\end{table}


==> table/tab_officehome.tex <==

\begin{table}
\caption{Subset of Table 1 (Columns 1-4 with "-A" added to Method names).}
\centering
\begin{tabular}{l|c|c|c}
\hline
Method & $\rightarrow$C & $\rightarrow$P & $\rightarrow$R \\
\hline
resnet-50-A & 46.7 & 68.6 & 74.9 \\
resnet-101-A & 48.7 & 69.5 & 76.1 \\
efficientnet-v2-s-A & 48.9 & 72.9 & 80.2 \\
efficientnet-v2-m-A & 54.0 & 74.0 & 80.4 \\
efficientnet-v2-l-A & 48.8 & 67.0 & 75.5 \\
\hline
vit-b-16-A & 50.9 & 74.7 & 80.2 \\
vit-b-32-A & 52.4 & 69.0 & 75.7 \\
vit-l-16-A & 47.0 & 74.2 & 79.1 \\
vit-l-32-A & 49.6 & 70.2 & 75.2 \\
vit-h-14-A & 76.5 & 91.1 & 91.5 \\
swin-t-A & 44.4 & 71.1 & 79.3 \\
swin-s-A & 52.4 & 75.8 & 81.7 \\
swin-b-A & 51.3 & 78.3 & 82.7 \\
swin-v2-t-A & 44.0 & 73.0 & 79.8 \\
swin-v2-s-A & 50.1 & 78.4 & 82.0 \\
swin-v2-b-A & 50.5 & 77.3 & 82.4 \\
\hline
\end{tabular}
\label{tab:subset-table1-A}
\end{table}




\begin{table}
\caption{Subset of Table 1 (Columns 1, 5-7 with "-C" added to Method names).}
\centering
\begin{tabular}{l|c|c|c}
\hline
Method & $\rightarrow$A & $\rightarrow$P & $\rightarrow$R \\
\hline
resnet-50-C & 54.4 & 63.7 & 65.6 \\
resnet-101-C & 54.3 & 65.6 & 67.0 \\
efficientnet-v2-s-C & 62.1 & 69.3 & 72.0 \\
efficientnet-v2-m-C & 62.9 & 72.8 & 73.4 \\
efficientnet-v2-l-C & 49.7 & 59.8 & 63.3 \\
\hline
vit-b-16-C & 66.5 & 75.0 & 75.7 \\
vit-b-32-C & 59.2 & 67.9 & 71.6 \\
vit-l-16-C & 61.4 & 73.3 & 74.2 \\
vit-l-32-C & 62.1 & 71.3 & 72.6 \\
vit-h-14-C & 87.5 & 91.7 & 90.2 \\
swin-t-C & 61.2 & 71.4 & 73.4 \\
swin-s-C & 66.0 & 74.4 & 76.0 \\
swin-b-C & 68.3 & 77.0 & 78.1 \\
swin-v2-t-C & 59.7 & 71.7 & 72.8 \\
swin-v2-s-C & 65.6 & 76.8 & 77.4 \\
swin-v2-b-C & 66.5 & 78.1 & 78.1 \\
\hline
\end{tabular}
\label{tab:subset-table1-cols-1-5-7-C}
\end{table}


\begin{table}
\caption{Subset of Table 1 (Columns 1, 8-10 with "-P" added to Method names).}
\centering
\begin{tabular}{l|c|c|c}
\hline
Method & $\rightarrow$A & $\rightarrow$C & $\rightarrow$R \\
\hline
resnet-50-P & 53.2 & 41.1 & 73.2 \\
resnet-101-P & 53.8 & 44.6 & 74.2 \\
efficientnet-v2-s-P & 62.3 & 47.2 & 80.1 \\
efficientnet-v2-m-P & 62.7 & 51.4 & 79.3 \\
efficientnet-v2-l-P & 61.2 & 51.8 & 79.8 \\
\hline
vit-b-16-P & 65.1 & 48.6 & 81.1 \\
vit-b-32-P & 56.9 & 47.4 & 76.2 \\
vit-l-16-P & 62.2 & 45.8 & 79.0 \\
vit-l-32-P & 60.8 & 50.2 & 77.3 \\
vit-h-14-P & 85.3 & 76.2 & 90.4 \\
swin-t-P & 62.6 & 42.5 & 79.8 \\
swin-s-P & 67.4 & 49.1 & 82.4 \\
swin-b-P & 68.7 & 49.6 & 82.7 \\
swin-v2-t-P & 61.6 & 44.5 & 79.7 \\
swin-v2-s-P & 65.4 & 49.6 & 81.2 \\
swin-v2-b-P & 66.3 & 49.3 & 81.5 \\
\hline
\end{tabular}
\label{tab:subset-table1-cols-1-8-10-P}
\end{table}

\begin{table}
\caption{Subset of Table 1 (Columns 1, 11-13 with "-R" added to Method names).}
\centering
\begin{tabular}{l|c|c|c}
\hline
Method & $\rightarrow$A & $\rightarrow$C & $\rightarrow$P \\
\hline
resnet-50-R & 66.4 & 48.1 & 78.0 \\
resnet-101-R & 68.1 & 50.0 & 79.2 \\
efficientnet-v2-s-R & 72.6 & 51.5 & 81.3 \\
efficientnet-v2-m-R & 73.3 & 55.0 & 82.2 \\
efficientnet-v2-l-R & 73.5 & 57.9 & 82.6 \\
\hline
vit-b-16-R & 71.0 & 48.0 & 80.8 \\
vit-b-32-R & 65.3 & 50.7 & 77.1 \\
vit-l-16-R & 68.0 & 46.3 & 80.9 \\
vit-l-32-R & 66.9 & 50.4 & 78.0 \\
vit-h-14-R & 89.7 & 78.5 & 94.7 \\
swin-t-R & 69.7 & 46.0 & 81.5 \\
swin-s-R & 73.0 & 51.2 & 84.7 \\
swin-b-R & 74.0 & 50.0 & 84.4 \\
swin-v2-t-R & 69.8 & 45.2 & 82.7 \\
swin-v2-s-R & 74.0 & 50.5 & 84.1 \\
swin-v2-b-R & 72.8 & 49.3 & 83.8 \\
\hline
\end{tabular}
\label{tab:subset-table1-cols-1-11-13-R}
\end{table}



==> table/tab_source_31_main.tex <==
\begin{table*}
\centering
\caption{Performance of source models on Office-31 tasks under Zoo-MSFDA setting.}
\begin{tabular}{|l|c|c|c|}
\hline
Method & A, D$\rightarrow$W & A, W$\rightarrow$D &D, W$\rightarrow$A \\
\hline
ResNet50 &72.1, 93.7  &79.1, 99.0  &62.9, 64.1\\
\hline
ResNet101 &74.5, 61.1  &79.1, 77.9  &28.2, 68.9  \\
\hline
EfficientNet\_V2\_S &68.1, 36.4  &73.0 , 53.8 &22.2, 43.4  \\
\hline
EfficientNet\_V2\_M &76.2, 27.2  &74.3, 67.7  &18.7, 44.6 \\
\hline
EfficientNet\_V2\_L &67.5, 40.6  &72.4, 73.0  &14.4, 33.4  \\
\hline
ViT\_B\_16 &85.3, 79.8  &86.1, 92.3 &53.7, 62.5 \\
\hline
ViT\_B\_32 &78.6, 77.7  &80.1, 92.1  &46.7, 66.9 \\
\hline
ViT\_L\_16  &82.9, 70.1  &82.7, 89.5 &50.8, 64.9 \\
\hline
ViT\_L\_32 &79.2, 69.4  &81.7, 84.5  &46.5, 55.6  \\
\hline
ViT\_H\_14 &92.7, 97.5  &92.1, 97.5  &79.6, 82.4  \\
\hline
Swin\_T &82.3, 61.6  &87.9, 85.7  &38.2, 56.9  \\
\hline
Swin\_S &85.9, 64.2  &86.7, 86.9  &47.2, 62.7  \\
\hline
Swin\_B &88.0, 64.1  &87.3, 85.7  &45.6, 59.7  \\
\hline
Swin\_L &91.8, 65.1  &92.9, 87.1  &46.9, 65.2  \\
\hline
Swin\_V2\_T &81.2, 66.1  &84.3, 92.2 &50.1, 62.9  \\
\hline
Swin\_V2\_S &85.5, 62.1  &87.8, 93.4  &45.6, 66.3  \\
\hline
Swin\_V2\_B &85.5, 62.3  &87.9, 78.1  &47.8, 55.5  \\
\hline
\end{tabular}
\label{tab:source_31main}
\end{table*}


==> table/tab_source_dn_main.tex <==
\begin{table*}
\centering
\scriptsize
%\resizebox{\textwidth}{!}{
\caption{Combined subset of Table 1}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Method & R$\rightarrow$I,P,S,C,Q & I$\rightarrow$R,P,S,C,Q  & P$\rightarrow$R,I,S,C,Q & S$\rightarrow$R,I,P,C,Q & C$\rightarrow$R,I,P,S,Q & Q$\rightarrow$R,I,P,S,C
\\
\hline
resnet-50 & 19.4,47.0,35.7,48.5,5.2
 & 44.7,29.2,25.4,31.4,2.0
 & 55.8,16.0,34.5,41.3,3.3
 & 44.4,13.5,34.7,49.1,11.7
 & 51.2,16.2,35.3,41.4,11.5
 & 3.4,1.0,1.4,7.2,8.8
 \\
\hline
resnet-101 & 21.3,49.3,37.8,50.0,6.8
 & 47.4,31.8,27.7,32.3,3.2 
 & 56.9, 18.0, 36.2,41.0,5.0
 & 50.0, 14.9, 38.5,50.2,13.0
 & 53.4,16.6,37.7,41.7,12.1
 & 3.7,0.5,1.1,8.6,6.2
 \\
\hline
efficientnet-v2-s 
& 22.4,52.7,41.6,53.5,7.9 
& 49.5,35.8,29.0,33.4,4.0
& 61.4,19.3,40.5,44.2,5.8
& 57.5,17.7,44.2,53.0,13.5 
& 58.3,18.8,41.6,43.4,12.9 
& 6.9,1.0,1.9,11.0,11.6
\\
\hline
efficientnet-v2-m 
& 22.5,53.4,43.0,54.9,7.6 
& 53.2,38.3,31.6,37.0,5.4
& 63.7,19.4,42.8,46.9,6.1 
& 58.6,17.5,46.0,55.4,13.7
& 59.3,19.2,42.2,45.2,12.7
& 10.3,2.0,3.9,12.4,17.0
\\
\hline
efficientnet-v2-l 
& 26.3,58.6,48.2,60.7,12,2 
& 48.5,35.4,29.3,36.0,6.0
& 66.7,22.5,43.6,51.8,9.0
& 59.2,18.2,46.8,56.3,16.3
& 60.1,20.0,43.7,45.8,15.6
& 3.7,0.7,0.9,11.4,6.0
\\
\hline
vit-b-16 
& 21.4, 50.6, 37.3,50.2,6.1 
& 53.2, 37.6, 30.1,36.3,4.1 
& 62.7, 19.3, 38.1,44.8,3.5
& 56.5,16.9,43.0,52.9,13.2
& 59.6,19.0,42.4,43.0,12.0
& 12.8,2.2,6.0,13.6,15.7
\\
\hline
vit-b-32 
& 18.1, 47.2, 34.6,48.0,6.1 
& 45.3, 31.7,25.1,30.7,2.6
& 58.3,16.3,34.7,41.3,3.7 
& 51.6,13.8,38.3,49.1,13.1
& 55.5,15.8,38.0,39.7,12.0
& 14.4,2.7,8.4,12.9,20.7
\\
\hline
vit-l-16 
& 20.4, 49.7, 35.1,48.8,4.9 
& 53.5, 35.7, 27.2, 34.9, 2.6
& 62.9,18.7,34.6,42.3,2.8 
& 54.6,15.1,40.7,50.8,12.7
& 58.9,18.7,39.8,40.1,10.1
& 14.0,2.8,6.8,10.1,15.5
\\
\hline
vit-l-32 
& 17.5, 47.6, 33.2,46.6,5.18 
& 43.4,31.1,23.4,29.1,2.6
& 58.0,16.1,32.5,39.8,1.9
& 52.2,13.9,39.5,48.0,12.3
& 56.3,15.7,38.9,38.3,12.2
& 19.2,3.9,11.0,15.8,23.9
\\
\hline
vit-h-14 
& 45.9,68.5,64.5,75.9,12.8 
& 75.5,60.1,57.9,67.2,12.3
& 75.3,40.4,60.7,67.9,8.6 
& 77.9,40.4,64.3,74.6,16.2
& 77.8,44.5,63.0,64.4,15.6
& 41.9,20.3,36.1,41.7,49.4
\\
\hline
swin-t 
& 19.4,47.7,33.3,45.0,5.9 
& 35.2,23.8,17.3,21.2,2.3
& 55.3,16.5,30.9,34.9,2.6 
& 48.6,13.3,36.8,42.9,8.3
& 50.8,14.4,33.7,34.9,7.8
& 15.2,3.9,8.4,13.1,20.8
\\
\hline
swin-s 
& 20.7,50.0,36.5,48.0,6.6
& 40.4,29.2,21.5,25.4,2.6 
& 58.2,18.6,34.9,39.0,3.3
& 53.9,15.6,42.2,47.0,10.5
& 54.7,17.1,38.3,38.1,9.3
& 20.8,5.6,13.1,17.7,25.1
\\
\hline
swin-b 
& 20.9, 50.0, 36.0,46.8,6.5
& 33.2,24.1,17.1,20.6,3.0
& 56.5,18.1,33.3,36.3,2.7
& 52.2,15.6,40.7,44.7,9.0
& 51.8,16.1,35.4,36.0,8.0
& 22.2,5.2,14.0,17.3,24.9
\\
\hline
swin-l 
& 29.4,61.2,50.9,62.4,10.5
& 50.9,40.2,33.4,37.3,6.8
& 67.4,26.3,45.5,52.4,6.5
& 67.0,23.8,51.5,62.0,14.8
& 66.8,25.3,50.4,51.3,12.9
& 33.0,10.9,22.9,29.5,39.2
\\
\hline
\end{tabular}%
%\label{tab:combined-subset-table1}
\end{table*}

==> table/tab_source_dn_main_new.tex <==
\begin{table*}
\centering
\tiny
%\resizebox{\textwidth}{!}{
\caption{Combined subset of Table 1}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Method & I, P, S, C, Q $\rightarrow$ R & R, P, S, C, Q $\rightarrow$ I & R, I, S, C, Q $\rightarrow$ P & R, I, P, C, Q $\rightarrow$ S & R, I, P, S, Q $\rightarrow$ C & R, I, P, S, C $\rightarrow$ Q
\\
\hline
ResNet50 &  44.7, 55.8, 44.4, 51.2, 3.4
 & 19.4, 16.0, 13.5, 16.2, 1.0
 & 47.0, 25.4, 34.7, 35.3, 1.4
 & 35.7, 25.4, 34.5, 41.4, 7.2
 & 48.5, 31.4, 41.3, 49.1, 8.8
 & 5.2, 2.0, 3.3, 11.7, 11.5
 \\
\hline
ResNet101 
& 47.4, 56.9, 50.0, 53.4, 3.7
& 21.3, 18.0, 14.9, 16.6, 0.5 
& 49.3, 31.8, 38.5, 37.7, 1.1
& 37.8, 27.7, 36.2, 41.7, 8.6
& 50.0, 32.3, 41.0, 50.2, 6.2
& 6.8, 3.2, 5.0, 13.0, 12.1
 \\
\hline
EfficientNet\_V2\_S
& 49.5, 61.4, 57.5, 58.3, 6.9
& 22.4, 19.3, 17.7, 18.8, 1.0
& 52.7, 35.8, 44.2, 41.6, 1.9
& 41.6, 29.0, 40.5, 43.4, 11.0
& 53.5, 33.4, 44.2, 53.0, 11.6
& 7.9, 4.0, 5.8, 13.5, 12.9
\\
\hline
EfficientNet\_V2\_M 
& 53.2, 63.7, 58.6, 59.3, 10.3 
& 22.5, 19.4, 17.5, 19.2, 2.0
& 53.4, 38.3, 46.0, 42.2, 3.9
& 43.0, 31.6, 42.8, 45.2, 12.4
& 54.9, 37.0, 46.9, 55.4, 17.0
& 7.6, 5.4, 6.1, 13.7, 12.7
\\
\hline
EfficientNet\_V2\_L 
& 48.5, 66.7, 59.2, 60.1, 3.7
& 26.3, 22.5, 18.2, 20.0, 0.7
& 58.6, 35.4, 46.8, 43.7, 0.9
& 48.2, 29.3, 43.6, 45.8, 11.4
& 60.7, 36.0, 51.8, 56.3, 6.0
& 12.2, 6.0, 9.0, 16.3, 15.6
\\
\hline
ViT\_B\_16 
& 53.2, 62.7, 56.5, 59.6, 12.8 
& 21.4, 19.3, 16.9, 19.0, 2.2 
& 50.6, 37.6, 43.0, 42.4, 6.0
& 37.3, 30.1, 38.1, 43.0, 13.6
& 50.2, 36.3, 44.8, 52.9, 15.7
& 6.1, 4.1, 3.5, 13.2, 12.0
\\
\hline
ViT\_B\_32 
& 45.3, 58.3, 51.6, 55.5, 14.4
& 18.1, 16.3, 13.8, 15.8, 2.7
& 47.2, 31.7, 38.3, 38.0, 8.4
& 34.6, 25.1, 34.7, 39.7, 12.9
& 48.0, 30.7, 41.3, 49.1, 20.7
& 6.1, 2.6, 3.7, 13.1, 12.0
\\
\hline
ViT\_L\_16 
& 53.3, 62.9, 54.6, 58.9, 14.0 
& 20.4, 18.7, 15.1, 18.7, 2.8
& 49.7, 35.7, 40.7, 39.8, 6.8 
& 35.1, 27.2, 34.6, 40.1, 10.1
& 48.8, 34.9, 42.3, 50.8, 15.5
& 4.9, 2.6, 2.8, 12.7, 10.1
\\
\hline
ViT\_L\_32 
& 43.4, 58.0, 52.2, 56.3, 19.2
& 17.5, 16.1, 13.9, 15.7, 3.9
& 47.6, 31.1, 39.5, 38.9, 11.0
& 33.2, 23.4, 32.5, 38.3, 15.8
& 46.6, 29.1, 39.8, 48.0, 23.9
& 5.2, 2.6, 1.9, 12.3, 12.2
\\
\hline
ViT\_H\_14 
& 75.5, 75.3, 77.9, 77.8, 41.9 
& 45.9, 40.4, 40.4, 44.5, 20.3
& 68.5, 60.1, 64.3, 63.0, 36.1 
& 64.5, 57.9, 60.7, 64.4, 41.7
& 75.9, 67.2, 67.9, 74.6, 49.4
& 12.8, 12.3, 8.6, 16.2, 15.6
\\
\hline
Swin\_T 
& 35.2, 55.3, 48.6, 50.8, 15.2 
& 19.4, 16.5, 13.3, 14.4, 3.9
& 47.7, 23.8, 36.8, 33.7, 8.4
& 33.3, 17.3, 30.9, 34.9, 13.1
& 45.0, 21.2, 34.9, 42.9, 20.8
& 5.9, 2.3, 2.6, 8.3, 7.8
\\
\hline
Swin\_S
& 40.4, 58.2, 53.9, 54.7, 20.8
& 20.7, 18.6, 15.6, 17.1, 5.6
& 50.0, 29.2, 42.2, 38.3, 13.1
& 36.5, 21.5, 34.9, 38.1, 17.7
& 48.0, 25.4, 39.0, 47.0, 25.1
& 6.6, 2.6, 3.3, 10.5, 9.3
\\
\hline
Swin\_B 
& 33.2, 56.5, 52.2, 51.8, 22.2
& 20.9, 18.1, 15.6, 16.1, 5.2
& 50.0, 24.1, 40.7, 35.4, 14.0
& 36.0, 17.1, 33.3, 36.0, 17.3
& 46.8, 20.6, 36.3, 44.7, 24.9
& 6.5, 3.0, 2.7, 9.0, 8.0
\\
\hline
Swin\_L 
& 50.9, 67.4, 67.0, 66.8, 33.0
& 29.4, 26.3, 23.8, 25.3, 10.9
& 61.2, 40.2, 51.5, 50.4, 22.9
& 50.9, 33.4, 45.5, 51.3, 29.5
& 62.4, 37.3, 52.4, 62.0, 39.2
& 10.5, 6.8, 6.5, 14.8, 12.9
\\
\hline
\end{tabular}%}
%\label{tab:combined\_subset\_Table1}
\end{table*}


==> table/tab_source_home_main.tex <==
\begin{table*}
\centering
\caption{Performance of source models on Office-Home tasks under Zoo-MSFDA setting.}
\begin{tabular}{|l|c|c|c|c|}
\hline
Method & A, C, P$\rightarrow$R & A, C, R$\rightarrow$P & A, P, R$\rightarrow$C & C, P, R$\rightarrow$A \\
\hline
ResNet50 & 74.9, 65.6, 73.2 & 68.6, 63.7, 78.0 & 46.7, 41.1, 48.1 & 54.4, 53.2, 66.4 \\
\hline
ResNet101 & 76.1, 67.0, 74.2 & 69.5, 65.6, 79.2 & 48.7, 44.6, 50.0 & 54.3, 53.8, 68.1 \\
\hline
EfficientNet\_V2\_S & 80.2, 72.0, 80.1 & 72.9, 69.3, 81.3 & 48.9, 47.2, 51.5 & 62.1, 62.3, 72.6 \\
\hline
EfficientNet\_V2\_M & 80.4, 73.4, 79.3 & 74.0, 72.8, 82.2 & 54.0, 51.4, 55.0 & 62.9, 62.7, 73.3 \\
\hline
EfficientNet\_V2\_L & 75.5, 63.3, 79.8 & 67.0, 59.8, 82.6 & 48.8, 51.8, 57.9 & 49.7, 61.2, 73.5 \\
\hline
ViT\_B\_16 & 80.2, 75.7, 81.1 & 74.7, 75.0, 80.8 & 50.9, 48.6, 48.0 & 66.5, 65.1, 71.0 \\
\hline
ViT\_B\_32 & 75.7, 71.6, 76.2 & 69.0, 67.9, 77.1 & 52.4, 47.4, 50.7 & 59.2, 56.9, 65.3 \\
\hline
ViT\_L\_16 & 79.1, 74.2, 79.0 & 74.2, 73.3, 80.9 & 47.0, 45.8, 46.3 & 61.4, 62.2, 68.0 \\
\hline
ViT\_L\_32 & 75.2, 72.6, 77.3 & 70.2, 71.3, 78.0 & 49.6, 50.2, 50.4 & 62.1, 60.8, 66.9 \\
\hline
ViT\_H\_14 & 91.5, 90.2, 90.4 & 91.1, 91.7, 94.7 & 76.5, 76.2, 78.5 & 87.5, 85.3, 89.7 \\
\hline
Swin\_T & 79.3, 73.4, 79.8 & 71.1, 71.4, 81.5 & 44.4, 42.5, 46.0 & 61.2, 62.6, 69.7 \\
\hline
Swin\_S & 81.7, 76.0, 82.4 & 75.8, 74.4, 84.7 & 52.4, 49.1, 51.2 & 66.0, 67.4, 73.0 \\
\hline
Swin\_B & 82.7, 78.1, 82.7 & 78.3, 77.0, 84.4 & 51.3, 49.6, 50.0 & 68.3, 68.7, 74.0 \\
\hline
Swin\_L & 90.3, 89.9, 91.9 & 87.4, 88.5, 91.5 & 71.5, 73.3, 73.4 & 83.9, 81.8, 85.0 \\
\hline
Swin\_V2\_T & 79.8, 72.8, 79.7 & 73.0, 71.7, 82.7 & 44.0, 44.5, 45.2 & 59.7, 61.6, 69.8 \\
\hline
Swin\_V2\_S & 82.0, 77.4, 81.2 & 78.4, 76.8, 84.1 & 50.1, 49.6, 50.5 & 65.6, 65.4, 74.0 \\
\hline
Swin\_V2\_B & 82.4, 78.1, 81.5 & 77.3, 78.1, 83.8 & 50.5, 49.3, 49.3 & 66.5, 66.3, 72.8 \\
\hline
\end{tabular}
\label{tab:source_main}
\end{table*}


==> table/tab_symbol.tex <==
\begin{table*}
\caption{Definition of the mathematical symbols.}
\centering

\begin{tabular}{l|c|c|c}
\hline
Symbol&Description &Symbol &Description\\
\hline
\multicolumn{4}{c}{Section 3}\\

\hline
$K$& the number of source domains&$C$& the number of categories\\
${D}_s^k$ & the $k$-th source domain& $\vert {D}_s^k\vert $ & the number of samples in $k$-th source domain\\
${D}_T$ & the target domain& $\vert {D}_T\vert $ & the number of samples in target domain\\
$x$/$x'$ & an image sample &$y$/$y'$ & the label of $x$/$x'$\\
$y_c$ & the  $c$-th element of the one-hot vector of $y$ &$N_r(x)$ & the $r$-nearest neighbors of $x$ \\
$A_r(x)$ & the $r$-adjacency group of $x$; $A_r(x)=x \cup N_r(x)$&$S_r(x)$ & $r$-adjacency-consistent score of $A_r(x)$\\

$h$/($h^k$) & the ($k$-th) source model& $f$/($f^k$) & the feature encoder of $h$/($h^k$)\\
$g$/($g^k$) & the classifier of $h$/($h^k$)& $\phi$/($\phi^k$) & the evidential head of $h$/($h^k$)\\

$p$/($p^k$) & the category probability of $x$ given by $h$/($h^k$)& $p'$ & the category probability of $x'$ given by $h$\\
$e$/($e^k$) & the evidence score of $x$ given by $h$/($h^k$)& $e'$ & the evidence score of $x'$ given by $h$\\
$\alpha$/($\alpha^k$) & the concentration parameter of $x$ given by $h$/($h^k$)& $\alpha'$ & the concentration parameter of $x'$ given by $h$\\
$S$/$S'$ & the total evidence of $x$/$x'$ given by $h$& $M$ & the max evidence of $x$ given by $h$\\
$p_c$/$e_c$/$\alpha_c$/$\alpha'_c$& the $c$-th element of $p$/$e$/$\alpha$/$\alpha'$&$max_c(\alpha_c)$/$max_c(\alpha'_c)$&the max element of $\alpha$/$\alpha'$\\

$\widetilde{\mu}$/$\widetilde{\mu}^k$& the EPU of $x$ given by $h$/$h^k$&$\hat{\mu}$/$\hat{\mu}^k$& the EAU within $A_r(x)$ given by $h$/$h^k$\\
$Ind$& the individual characteristic &$Int$& the interactive characteristic\\
$\dot{\alpha}_c$& formulated by $y_c+(1-y_c)\alpha_c$&$\mathbb{E}$&the expectation function\\
$Mul(.)$/$Dir(.)$&the Multinomial/Dirichlet distribution&$\beta(.)$ & the $C$-dimensional Multinomial Beta function\\
$\mathbb{I}$& the indicator function&$I$ & the Regularized Incomplete Beta function\\

\hline
\multicolumn{4}{c}{Section 4}\\
\hline
$Ip$& the instance preference of $x$ &$Ip^k$& the preference of $x$ to the $h^k$ \\
$s$& the index of the strong source model&$k;k\neq s$&  the index of complementary source model\\
$\Omega^{k}$&the consultation dictionary of $h^s$ to $h^k$ ($k\neq s$) &$\Omega^{k}[x]$& the value of $\Omega^{k}$ specific to $x$\\
$p^{fk}$ & the fusion of $p^{k}$ and $p^s$ &$\alpha^{fk}$ & the fusion of $\alpha^{k}$ and $\alpha^s$\\

$x_i$ & the $i$-th image sample from target domain & $p^k(x_i)$/$f^k(x_i)$& the category probability/feature of $x_i$ given by $h^k$\\
$F_i$& the concatenation of $\{f^k(x_i)\}_{k=1}^{K}$ &$\mathcal{F}$& the feature bank $\{F_1, F_2, ..., F_{\vert D_T\vert}\}$\\
$\tau$& the self-adaptive category-aware threshold& $\tau_c$& the threshold for category $c$\\
$A_r(x_i)$ &the $r$-adjacency group of $x_i$ &$\hat{y}_i$& the pseudo label of $x_i$\\
$Aug(x_i)$& the data augmentation of $x_i$&$\hat{\mu}_i$& the EAU within $A_r(x_i)$ given by $h^s$\\

$D_{sec}$& the secure groups in target domain &$\vert D_{sec} \vert $ & the number of samples in $D_{sec}$\\
$D_{ris}$& the risky groups in target domain&$\vert D_{ris} \vert $ & the number of samples in $D_{ris}$\\

\hline
\end{tabular}
%}
\label{tab_sym}
\end{table*}
